A mix of long-duration hydrogen and thermal storage enables large-scale electrified heating in a renewable European energy system

Hydrogen-based long-duration electricity storage (LDES) is a key component of renewable energy systems to deal with seasonality and prolonged periods of low wind and solar energy availability. In this paper, we investigate how electrified heating with heat pumps impacts LDES requirements in a fully renewable European energy system, and which role thermal storage can play. Using a large weather dataset of 78 weather years, we find that electrified heating significantly increases LDES needs, as optimal average energy capacities more than quadruple across all weather years compared to a scenario without electrified heating. We attribute 75% of this increase to a leverage effect, as additional electric load amplifies storage needs during times of low renewable availability. The remaining 25% are the result of a compound effect, where exceptional cold spells coincide with periods of renewable scarcity. Furthermore, heat pumps increase the variance in optimal storage capacities between weather years substantially because of demand-side weather variability. Long-duration thermal storage attached to district heating networks can reduce LDES needs by on average 36%. To support and safeguard wide-spread heating electrification, policymakers should expedite the creation of adequate regulatory frameworks for both long-duration storage types to de-risk investments in light of high weather variability.

==> tables/regression_table.tex <==
\begin{tabular}{lrrrr}
\toprule
                                          & \multicolumn{4}{c}{Dependent variable: Heat-related LDS increase, TWh} \\
\cmidrule(lr){2-5}
                                          &             (1) &             (2) &             (3) &              (4) \\
\midrule
(Intercept)                               &      161.252*** &      161.252*** &      161.252*** &       161.252*** \\
                                          &         (5.736) &         (5.601) &         (5.082) &          (2.880) \\
Total heat demand, TWh                    &        0.187*** &        0.167*** &          -0.022 &          -0.066* \\
                                          &         (0.024) &         (0.025) &         (0.051) &          (0.029) \\
Total renewable generation potential, TWh &                 &         -0.076* &        -0.106** &         0.105*** \\
                                          &                 &         (0.035) &         (0.033) &          (0.025) \\
Cold spell excess heat demand , $TWh_{th}$    &                 &                 &        0.000*** &           0.000* \\
                                          &                 &                 &         (0.000) &          (0.000) \\
Max combined residual load, TWh           &                 &                 &                 &         0.500*** \\
                                          &                 &                 &                 &          (0.040) \\
\midrule
Obs.                                      &              78 &              78 &              78 &               78 \\
Adj. R2                                   &           0.444 &           0.469 &           0.563 &            0.860 \\
\bottomrule
\end{tabular}
